Unimodal Distributions for Ordinal Regression

In many real-world prediction tasks, class labels contain information about the relative order between labels that are not captured by commonly used loss functions such as multicategory cross-entropy. Recently, the preference for unimodal distributions in the output space has been incorporated into models and loss functions to account for such ordering information. However, current approaches rely on heuristics that lack a theoretical foundation. Here, we propose two new approaches to incorporate the preference for unimodal distributions into the predictive model. We analyse the set of unimodal distributions in the probability simplex and establish fundamental properties. We then propose a new architecture that imposes unimodal distributions and a new loss term that relies on the notion of projection in a set to promote unimodality. Experiments show the new architecture achieves top-2 performance, while the proposed new loss term is very competitive while maintaining high unimodality.

==> tables/results-lambda.tex <==

\begin{tikzpicture}[font=\footnotesize]
\begin{groupplot}[
    group style={
        group name=myplots,
        columns=2,
        horizontal sep=5pt,
    },
    grid=both,
    height=5cm,
    table/col sep=space,
    scale only axis=true,  % this is so we can make them proportional
    xticklabel={\pgfmathparse{\tick}\pgfmathprintnumber{\pgfmathresult}\%},
    yticklabel={\pgfmathparse{\tick}\pgfmathprintnumber{\pgfmathresult}\%},
    legend pos=south east,
    legend cell align={left},
    legend style={draw=none, fill=none},
]
\nextgroupplot[
    width=0.33*7cm,
    axis y line=left,
    axis line style={-},
    xmin=0, xmax=25,
    ymin=0, ymax=100,
    xtick={0,20},
    ylabel={\%Unimodal},
]
\addplot[
    only marks,
    scatter,
    scatter/classes={1={mark=o}, 2={mark=halfcircle}, 3={fill=gray}, 4={mark=otimes}},
    scatter src=explicit,
    visualization depends on=\thisrow{lambda}\as\lambda,
    scatter/@pre marker code/.append style={/tikz/mark size=(log10(\lambda)+4)/2},
] table[x=acc, y=unimodality, meta=dataset] {data.csv};

\nextgroupplot[
    width=0.66*7cm,
    axis y line=right,
    axis line style={-},
    xmin=55, xmax=100,
    ymin=0, ymax=100,
    yticklabels={},
    xtick={60,80,100},
]
\addplot[
    only marks,
    scatter,
    scatter/classes={1={mark=o}, 2={mark=halfcircle}, 3={fill=gray}, 4={mark=otimes}, 5={mark=square}},
    scatter src=explicit,
    visualization depends on=\thisrow{lambda}\as\lambda,
    scatter/@pre marker code/.append style={/tikz/mark size=(log10(\lambda)+4)/2},
] table[x=acc, y=unimodality, meta=dataset] {data.csv};

\draw[black, fill=white] (56, 2) rectangle (100, 48);
\legend{ICIAR, DHCI, FGNET, SMEAR2005, FOCUSPATH}

\end{groupplot}
\node[fit=(myplots c1r1)(myplots c2r1)](mygroup){};
\node[below=4mm of mygroup.south] {Accuracy};

\coordinate (lambda1) at ([xshift=-12em, yshift=21.5mm]myplots c2r1.south east);
\coordinate (lambda2) at ([xshift=-12em, yshift=18.5mm]myplots c2r1.south east);
\coordinate (lambda3) at ([xshift=-12em, yshift=15.5mm]myplots c2r1.south east);
\coordinate (lambda4) at ([xshift=-12em, yshift=12.5mm]myplots c2r1.south east);
\coordinate (lambda5) at ([xshift=-12em, yshift=9.5mm]myplots c2r1.south east);
\coordinate (lambda6) at ([xshift=-12em, yshift=6.5mm]myplots c2r1.south east);
\coordinate (lambda7) at ([xshift=-12em, yshift=3.5mm]myplots c2r1.south east);

\draw (lambda1) circle (4.2pt); \node[right=2mm of lambda1, font=\footnotesize] {$\lambda=10^3$};
\draw (lambda2) circle (3.5pt); \node[right=2mm of lambda2, font=\footnotesize] {$\lambda=10^2$};
\draw (lambda3) circle (3pt); \node[right=2mm of lambda3, font=\footnotesize] {$\lambda=10$};
\draw (lambda4) circle (2.1pt); \node[right=2mm of lambda4, font=\footnotesize] {$\lambda=1$};
\draw (lambda5) circle (1.5pt); \node[right=2mm of lambda5, font=\footnotesize] {$\lambda=10^{-1}$};
\draw (lambda6) circle (1pt); \node[right=2mm of lambda6, font=\footnotesize] {$\lambda=10^{-2}$};
\draw (lambda7) circle (0.6pt); \node[right=2mm of lambda7, font=\footnotesize] {$\lambda=10^{-3}$};


% discontinuity axis drawing (below)
\draw ([xshift=-1mm, yshift=-2mm]myplots c1r1.south east) -- ([xshift=1mm, yshift=2mm]myplots c1r1.south east);
\draw ([xshift=-1mm, yshift=-2mm]myplots c2r1.south west) -- ([xshift=1mm, yshift=2mm]myplots c2r1.south west);
% discontinuity axis drawing (above)
\draw ([xshift=-1mm, yshift=-2mm]myplots c1r1.north east) -- ([xshift=1mm, yshift=2mm]myplots c1r1.north east);
\draw ([xshift=-1mm, yshift=-2mm]myplots c2r1.north west) -- ([xshift=1mm, yshift=2mm]myplots c2r1.north west);

\end{tikzpicture}
